SAGAbg II: the Low-Mass Star-Forming Sequence Evolves Significantly Between 0.05<z<0.21

The redshift-dependent relation between galaxy stellar mass and star formation rate (the Star-Forming Sequence, or SFS) is a key observational yardstick for galaxy assembly. We use the SAGAbg-A sample of background galaxies from the Satellites Around Galactic Analogs (SAGA) Survey to model the low-redshift evolution of the low-mass SFS. The sample is comprised of 23258 galaxies with H$\alpha$-based star formation rates (SFRs) spanning $6<\log_{10}(\rm M_\star/[M_\odot])<10$ and $z<0.21$ ($t<2.5$ Gyr). Although it is common to bin or stack galaxies at $z \lesssim 0.2$ for galaxy population studies, the difference in lookback time between $z=0$ and $z=0.21$ is comparable to the time between $z=1$ to $z=2$. We develop a model to account for both the physical evolution of low-mass SFS and the selection function of the SAGA survey, allowing us to disentangle redshift evolution from redshift-dependent selection effects across the SAGAbg-A redshift range. Our findings indicate significant evolution in the SFS over the last 2.5 Gyr, with a rising normalization: $\langle {\rm SFR}({\rm M_\star=10^{8.5} M_\odot)}\rangle(z)=1.24^{+0.25}_{-0.23}\ {\rm z} -1.47^{+0.03}_{-0.03}$. We also identify the redshift limit at which a static SFS is ruled out at the 95% confidence level, which is $z=0.05$ based on the precision of the SAGAbg-A sample. Comparison with cosmological hydrodynamic simulations reveals that some contemporary simulations under-predict the recent evolution of the low-mass SFS. This demonstrates that the recent evolution of the low-mass SFS can provide new constraints on the assembly of the low-mass Universe and highlights the need for improved models in this regime.

==> SAGAbgShared/SFR_Mstar_first.tex <==

\subsection{Star Formation Rates}
We estimate star formation rates following 
\cite{calzetti2013} for a Kroupa IMF:
\begin{equation}\label{e:lha2sfr}
  \text{SFR} = \beta_c {F^{\rm e}_{\text{\halpha{}}} (4\pi d_L^2)}.
\end{equation}
where $\beta_c=5.5\times10^{-42}\ M_\odot\text{ erg}^{-1}$ is a scaling factor that 
depends on the adopted IMF and evolutionary library, as well as GMC-scale 
assumptions about ionizing photon leakage from \HII{} regions and ionizing photon 
absorption by dust. We correct for optical extinction from a fit to the Balmer decrement; we 
show the distribution of $A_V$ for the same as a function of stellar mass in \autoref{f:extinctionsample}
These conversions 
between \halpha{} luminosity and a star formation rate, as well 
as the interpretation of that star formation rate as the average over some time period $T$ (where $T$ is typically cited as $5-10$ Myr), hinges upon the 
assumption that the star formation rate is constant over $T$. To test the sensitivity of $\beta$ on $T$, 
we compute $\beta(T)$ using the ionizing photon rate for a~\cite{kroupa2001} IMF 
using \textsf{Starburst99} \citep{leitherer1999}. We find that the $\beta(T)$
change in $\beta(T)$ for $T>6$ Myr is small, where 
$\log_{10}[\beta(T=6\text{ Myr})/\beta(T=10\text{ Myr})]=-0.013$. We find 
a $\beta(6\text{ Myr}) = 5.01\times10^{-42}\ M_\odot\text{ erg}^{-1}$, but adopt
the~\cite{calzetti2013} value because of the minimal offset and its widespread 
use in the literature. 



\subsection{Stellar Masses}
We follow the stellar mass prescription established for the SAGA survey 
by \cite{mao2021} and estimate our stellar masses as:
\begin{equation}
  \log_{10}\left( \frac{M_\star}{M_\odot} \right) = 1.254 + 1.098(g-r)_{\rm rf} - 0.4 M_{r,\rm rf}.
\end{equation}
The ``rf'' subscript above indicates restframe measurements. 

This relation is an adaptation of the~\cite{bell2003} mass-to-light and color relation that has been calibrated for the
SAGA sample via a comparison to stellar mass estimates in the SAGA mass range.
As in~\cite{mao2021} and \citetalias{otherpaper}, we assume an uncertainty of 0.2 dex for our stellar mass estimates. 

Although the color-mass relation that we use in this work has been calibrated 
for our stellar mass range by \cite{mao2021}, it is worth noting that color-mass relations for low mass galaxies are often extrapolations from relations calibrated at 
higher mass. To make sure that the SAGA color-mass relation is applicable to our 
background galaxies, we compare the publically available stellar masses produced 
by the GAMA survey via SED fitting \citep[\textsf{StellarMassesLambdarv20},][]{taylor2011} with the stellar masses that we would assign 
to these galaxies using the above color-mass relation. Here we use the same photometry 
as the GAMA SED-fit stellar masses to exclude any additional systematic differences 
that could result from a comparison of different photometric methods. 

We find that, over 6.8$<$\logmstar[$\leq$10], there is an average offset of 
$\Delta$\logmstar[$=0.01$] between the two methods. However, there is a significant 
positive slope to the relation between $\Delta$\logmstar[] and \logmstar[] such that 
lower stellar masses show a larger discrepancy, up to a median 
$\Delta$\logmstar[$=0.13$]
at \logmstar[$<7.2$]. This slope is significant and 
is in line with ongoing work to inspect the fidelity of 
photometric stellar mass estimates at low stellar masses \citeprep{de los Reyes}; for 
the scope of this analysis, however, we will simply emphasize that this offset is 
below our assumed uncertainty in stellar mass of $0.2$ dex.


==> SAGAbgShared/SFR_Mstar_second.tex <==
\subsection{Stellar Masses and Star Formation Rates}
We adopt the stellar mass and star formation rate estimates that were established and validated in
\citetalias{otherpaper}. Briefly, this yields 
\halpha{}-based star formation rates of:
\begin{equation}\label{e:lha2sfr}
  \text{SFR} = \beta_c {F^{\rm e}_{\text{\halpha{}}} (4\pi d_L^2)},
\end{equation}
where $\beta_c=5.5\times10^{-42}\ M_\odot\text{ erg}^{-1}$ is the scalar factor introduced by \cite{calzetti2000}.
We follow \citetalias{otherpaper} and \cite{mao2021} to estimate stellar masses based on a color-mass relation:
\begin{equation}
  \log_{10}\left( \frac{M_\star}{M_\odot} \right) = 1.254 + 1.098(g-r)_{\rm rf} - 0.4 M_{r,\rm rf}.
\end{equation}
Here, the ``rf'' subscript above indicates restframe measurements. 

==> SAGAbgShared/assumptions_first.tex <==
We justify the first assumption as follows: more distant galaxies will have lower \halpha{} fluxes for a given \halpha{} luminosity, and redshift-induced observational reddening in our bands of interest indicates that we will tend to select bluer and more star-forming galaxies at fixed stellar mass and increasing redshift. Due to our effective photometric selection 
preferring blue galaxies, the first assumption should be naturally satisfied. 

The second assumption should be generally satisfied given our relative completeness assumption and the fact that the rate of stellar mass accretion is small compared to our stellar mass range, though there will be some galaxies that enter or leave the selection area (e.g. stellar mass exceeds $M_\star =10^{10}M_\odot$, quenching). 
Our stellar mass range is selected such that 
self-quenching in the past \tlbmax{} should be a marginal effect -- in the field,
$\sim 5\%$ of galaxies at \logmstar{}$=9.75$ and $<1\%$ of those at \logmstar{}$<8.5$ are quenched. 

We do not make an explicit environmental cut on our sample, and so one should consider whether the divergent evolution of field and satellite galaxies would affect our analysis. Because we select for star-forming galaxies by dint of our line detection criterion and low-mass, blue galaxies by dint of our photometric selection, we find that our satellite fraction is both small and constant.
We show in 
\autoref{s:appendix:environment} that our
satellite fraction is consistent with $\approx 5\%$ across all redshift bins.

There should also be galaxies at the high stellar
mass end of our sample that will reach \logmstar{$>10$} by our $z\sim0$ reference sample. However, our comparison should not be affected by these galaxies given that we are performing a relative optimization (and by construction, none of our models will produce galaxies that exceeded \logmstar[$=10$] at high redshift and became \logmstar[$<10$] at $z\approx0$).

Finally, due to a declining stellar-to-halo relation, 
low-mass galaxies are not generally expected to accrete significant stellar mass via minor mergers \citep{purcell2007, brook2014}. 
Though major mergers between dwarf galaxies do occur, these are relatively rare at low redshift, with
pair and merger searches yielding an expected merger incidence of a few percent \citep{stierwalt2015,besla2018, kadofong2020a}. We thus expect stellar mass build-up due to accretion to be 
negligible in the past \tlbmax{} for our sample on a statistical level. 

==> SAGAbgShared/lines_first.tex <==
The first step of this process is to measure fluxes of the relevant lines in our
sample. The most important lines for our analysis in this paper series are \halpha, \hbeta, 
\ftst, \foos{}, \oiidoublet, \sttoB, and \sttoR. We also fit a wider set of lines 
including the density-sensitive pair \ionline{S}{2}{6717} and \ionline{S}{2}{6731}, and a set of 
weaker non-oxygen auroral lines (\ionline{N}{2}{5755}, \ionline{S}{2}{4069}, 
\ionline{S}{2}{4077}). A full accounting of the lines fit for this analysis will be provided as an value-added catalog in a
forthcoming work \citeprep{Mao}.

We fit our emission lines and Balmer absorption features simultaneously; we
allow the amplitude and position to vary for each line but assume that all the emission lines can be well-described 
by a Gaussian profile of the same width $\sigma_{em}$. The Balmer absorption features are also fit as an ensemble of 
Gaussian profiles wherein we require that the ratio between the equivalent width of each absorption feature and the
equivalent width of the H$\beta$ absorption feature is held to be unity for H$\gamma$ and H$\delta$, and 
0.5 for H$\alpha$ (i.e. $\rm EW_{H\alpha} = 0.5 EW_{H\beta}$). This relationship is chosen based on the models of 
\cite{gonzalezdelgado1999}; we adopt a strict assumption here because the H$\alpha$ absorption is not spectrally 
resolved and is therefore degenerate with the emission component. We approximate the
continuum local to each emission line as a constant value, and hold the continuum flux of lines separated by less than
140\AA{} to be equal. 
We infer the properties of the all the emission line profiles in each 
SAGA spectra simultaneously via the Markov Chain Monte Carlo ensemble sampler implemented in \textsf{emcee}
\citep{emcee}.

Our approach allows us to straightforwardly incorporate our knowledge of atomic physics into 
the line profile fitting by including this information into our formulation of the prior. In particular, we have strong 
constraints on the minimum allowable flux ratio of lines originating from the same species 
wherein the redder line is in the numerator. As an example, let us consider the flux ratio between \halpha{} and \hbeta{}, 
i.e. the Balmer decrement.
For a gas at \nelec{}$=10^3$ \cc{} and \te{}$=10^4$ K, the intrinsic flux ratio between \halpha{} and \hbeta{} should 
be 2.86. In the presence of reddening from dust, the observed flux ratio may be larger than this value (but not smaller). 
We thus adopt a sigmoid prior
\begin{equation}
  \rm Pr(A_{H\alpha}, A_{H\beta}) = (1 + e^{-k(A_{H\alpha}/A_{H\beta} - \tilde A_{H\alpha,H\beta}b)})^{-1}
\end{equation} 
where
$k=30$ and $b=0.925$ are the shape parameters of the sigmoid function, $\tilde A_{H\alpha,H\beta}$ is the intrinsic
flux ratio (here assumed to be 2.86), and $\rm A_{H\alpha}$ and $\rm A_{H\beta}$ are the
amplitudes of the \halpha{} and \hbeta{} lines, taking advantage of the fact that the ratio of the fluxes will be 
equal to the ratio of the amplitudes when the linewidth is equal. Note that the prior allows for, but is weighted against, 
line ratios somewhat below the assumed minimum intrinsic ratio.
The same exercise can be performed with the
other lines in the spectrum; we assume sigmoid priors with the following assumed intrinsic ratios:
\begin{itemize}[itemsep=-0.5mm]\vspace{-2mm}
  \item[] $\tilde A_{H\alpha,H\gamma}=6.11$ 
  \item[] $\tilde A_{H\alpha,H\delta}=11.06$ 
  \item[] $\tilde A_{[OIII]5007,[OIII]4959}=2.98$ 
  \item[] $\tilde A_{[OIII]5007,[OIII]4363}=6.25$ 
  \item[] $\tilde A_{[SII]4077,[SII]4069}=6.25$  
\end{itemize}
based off of the minimum intrinsic line ratio for a reasonable ($10^2\lesssim T\lesssim 10^5$ K) range in temperature as 
computed by the package \textsf{pyneb}. 

We adopt a simple Gaussian likelihood over our model parameters:
% residsq = (self.model.evaluate ( self.wave )  -  self.flux)**2        
% inner = -0.5*np.sum(residsq / self.u_flux**2 + np.log(2.*np.pi*self.u_flux**2) ) 
\begin{equation}
  \ln\mathcal{L}(\vec F_\lambda | \vec \theta_\ell) = -\frac{1}{2}\sum_{i}{\left[\frac{{\left( \hat F_\lambda(\lambda_i,\vec \theta_\ell) - F_{\lambda,i} \right)}^2}{\sigma_{F_{\lambda,i}}^2} +
  \ln{\left( 2 \pi \sigma_{F_\lambda,i}^2\right)}\right]},
\end{equation}   
where the index refers to the index of the resolution element, $\hat F_\lambda(\lambda_i)$ and $F_{\lambda,i}$ are the predicted and observed specific fluxes in that resolution element, respectively, and $\sigma_{F_\lambda}$ is the uncertainty in the specific flux. 
The observed spectrum is thus simply $\vec F_\lambda = \{F_{\lambda,0}, F_{\lambda,1} ... F_{\lambda, M}\}$ for $M$ resolution elements.
The vector $\vec \theta_\ell$ is of length $2N_{\rm em} + N_{\rm cont} + 3$; $\vec \theta_\ell$ describes the parameters of the line model. Here $N_{\rm em}\leq\nemission{}$ is the number of emission lines fit and $N_{\rm cont}\leq \ncontinuum$
is the number of continuum regions fits. The numbers here are given as upper limits 
because lines that are redshifted beyond $\lambda=8000\text{ \AA}$ are excluded from 
the model.
There are then an additional 3 parameters: $\sigma_{\rm em}$, the width of the emission lines, $\text{EW}_{\rm abs}$, the 
equivalent width of the Balmer lines, and $\sigma_{\rm abs}$, the width of the (Balmer)
absorption lines.

Because some of the lines that we fit are quite weak (at maximum $\sim 10\%$ the flux of \halpha{} and
\ionline{O}{3}{5007}), we visually inspect each galaxy in which the inference predicts a less than 16\% chance that the auroral oxygen lines could originate from stochastic fluctuations to ensure that the measured features are not observational artifacts such as residuals from sky subtraction.
Finally, in \autoref{s:appendix:fluxcalibration} we test both our flux calibration and line measurement methods against published GAMA survey 
results to verify that our methodology is consistent with established literature methods.

==> SAGAbgShared/lines_second.tex <==

%sqFor completeness, however, we will summarize the measurement methodology below. 
We adopt a Gaussian profile with a fixed line width, $\sigma_{\rm em}$, for the 
emission lines and an additional Gaussian profile with a fixed equivalent width, $\rm EW_{abs}$, for the Balmer 
absorption features. Because the \halpha{} absorption and emission are generally not resolved in our 
spectra, we adopt a fixed $EW_{abs} = 2 \rm EW_{H\alpha} = EW_{H\beta}$ following \citep{gonzalezdelgado1999}.
We approximate the local continuum as a constant value and allow the line centroids to shift up to $\Delta \lambda = 1.5 \rm \AA$ to account for minor inaccuracies in our 
relative wavelength solution.

We infer best-fit line parameters using the Markov Chain Monte Carlo package \textsf{emcee} \citep{emcee}.
As detailed in \citetalias{otherpaper}, this approach allows us to easily incorporate our understanding of atomic physics into our line fits by imposing a prior over line flux ratios of the same species. 
Because lines at larger wavelengths should also be relatively less reddened from to extinction in the galaxy, 
we place a one-sided prior of the form:
\begin{equation}
  \rm Pr(F_{\lambda_r}, F_{\lambda_b}) = (1 + e^{-k(F_{\lambda_r}/F_{\lambda_b} - (F_{\lambda_r}/F_{\lambda_b})_{\rm intr} )})^{-1}
\end{equation} 
where $k=30$ and $b=0.925$ are the shape parameters of the sigmoid function, $F_{\lambda_r}$ is the line flux of the 
redder line, $F_{\lambda_b}$ is the line flux of the bluer line, and $(F_{\lambda_r}/F_{\lambda_b})_{\rm intr}$ is 
minimum intrinsic line ratio expected over the temperature range $10^3<T<10^5$ K and density range $10<n_e<10^3$ 
cm$^{-3}$. This prior allows for, but is weighted against, line flux ratios lower than $(F_{\lambda_r}/F_{\lambda_b})_{\rm intr}$.
We adopt a simple Gaussian likelihood over our model parameters:
\begin{equation}
  \ln\mathcal{L}(\vec F_\lambda | \vec \theta_\ell) = -\frac{1}{2}\sum_{i}{\left[\frac{{\left( \hat F_\lambda(\lambda_i,\vec \theta_\ell) - F_{\lambda,i} \right)}^2}{\sigma_{F_{\lambda,i}}^2} +
  \ln{\left( 2 \pi \sigma_{F_\lambda,i}^2\right)}\right]},
\end{equation}   
where the index refers to the index of the resolution element, $\hat F_\lambda(\lambda_i)$ and $F_{\lambda,i}$ are the predicted and observed specific fluxes in that resolution element, respectively, and $\sigma_{F_\lambda}$ is the uncertainty in the specific flux. 
The observed spectrum is thus simply $\vec F_\lambda = \{F_{\lambda,0}, F_{\lambda,1} ... F_{\lambda, M}\}$ for $M$ resolution elements.
The vector $\vec \theta_\ell$ is of length $2N_{\rm em} + N_{\rm cont} + 3$; $\vec \theta_\ell$ describes the parameters of the line model. Here $N_{\rm em}\leq\nemission{}$ is the number of emission lines fit and $N_{\rm cont}\leq \ncontinuum$
is the number of continuum regions fits. The numbers here are given as upper limits 
because lines that are redshifted beyond $\lambda=8000\text{ \AA}$ are excluded from 
the model.
There are then an additional 3 parameters: $\sigma_{\rm em}$, the width of the emission lines, $\text{EW}_{\rm abs}$, the 
equivalent width of the Balmer lines, and $\sigma_{\rm abs}$, the width of the Balmer
absorption features.

==> SAGAbgShared/observational_constraints_first.tex <==
Finally, we must also include the effects of our selection function. This includes both the photometric selection that we described in \autoref{s:sample:photometric}, and the requirement for an emission line detection.
We compute the expected $g-r$ color at luminosity distance $d_{L}(t_{i+1})$ and effective on-sky radius at angular diameter distance $d_{A}(t_{i+1})$ by computing reverse k-corrections directly from the spectra; we require that the galaxy have an apparent magnitude of $m_r<21$ and 
remain ``observed'', which we will presently describe, at $t_{i+1}$. 

The effective SAGA targeting scheme is based upon the apparent (galactic extinction-corrected) 
r-band magnitude of the galaxy, its effective r-band surface brightness, and its
$g-r$ color \citep{mao2021}.  
In order to quantify the probability that a devolved galaxy would have
been selected for observation, we simply measure the fraction of galaxies that have observations from SDSS, GAMA,
or SAGA AAT/MMT as a function of their (binned) photometric properties. This is done in three dimensions; 
for visualization purposes we show the projected targeted fraction for our photometric parameter space 
in \autoref{f:targeting}. In each panel group, the upper panels show the distribution of all possible 
targets (left, red) and the targeted galaxies (right, blue). 
The main panel shows the fraction of galaxies targeted
as a function of their photometric properties, where
the size of the box corresponds inversely to the uncertainty on the measured fraction assuming a binomial 
distribution. One can clearly see the imprint of the photometric selection described in~\cite{mao2021}, wherein galaxies that are bluer and lower surface brightness are more 
likely to have been observed. 

At each timestep, we compute the observed-frame $r$-band magnitude, $r$-band surface brightness, and $g-r$ color of each devolved galaxy. Because there is uncertainty associated with our measurement of the targeted fraction, 
at each timestep we estimate the targeted fraction by drawing from a uniform distribution bounded by the 95\% 
confidence interval. 
We then sample from a uniform distribution bounded by zero and unity to and the galaxy is flagged as observed if the targeted probability exceeds the drawn number.


For each spectrum we additionally estimate the \halpha{} detection limit as three times the standard deviation of the blank spectrum within $140(1+z_{i+1})$ \AA{} of \halpha{} (we mask \halpha{}, \ionline{N}{2}{6548}, and \ionline{N}{2}{6583}). We convert SFR$(t_{i+1})$ to an \halpha{} flux using the inverse of \autoref{e:lha2sfr}, i.e.:
\begin{equation}
  F_{\text{\halpha{}}}(t_{i+1}) = \frac{\text{SFR}(t_{i+1})/[M_\odot\ \rm yr^{-1}]}{5.5\times10^{-42}} \frac{1}{4\pi d_L^2(z_{i+1})}.
\end{equation}
To be flagged as observable, we require that $F_{\text{\halpha{}}}(t_{i+1})$ exceed the 
$3\sigma$ detection limit defined above.

==> SAGAbgShared/observational_constraints_second.tex <==
As in \citetalias{otherpaper}, we apply the effect of our 
selection function to evaluate whether our retrogressed galaxies would be 
observable (that is, whether the SAGA survey would have suceeded in obtaining a secure redshift) at a given lookback time. As we have done earlier in the manuscript, we will summarize the salient points of the selection function here but note to the reader of \citetalias{otherpaper} that the content is the same between the two articles.

The SAGA spectroscopic targeting scheme is based upon the apparent $r$-band magnitude, $r$-band surface brightness, and $g-r$ color of the target. In \citetalias{otherpaper}, we determined the probability that a potential target would be targeted in the \sagabg{} sample as a function of its photometric properties. The photometric properties of each retrogressed galaxy are then determined at the retrogressed redshift, and the galaxy is stochastically targeted with the prescribed targeting probability.

For each spectrum we additionally estimate the \halpha{} detection limit;
to be flagged as observable, we require that the retrogressed galaxy be targeted and that its \halpha{} flux at the retrogressed redshift exceeds the 
$3\sigma$ detection limit defined above.

==> SAGAbgShared/spectra_first.tex <==
\subsection{\sagabg{} Spectra}\label{s:methods:spectra}
Measuring star formation rates from \halpha{} luminosities and gas-phase metallicites from temperature-sensitive oxygen line flux ratios requires flux-calibrated spectra.
We find that the relative flux calibration of the SAGA AAT and MMT spectra, particularly those spectra from \aat{}, degrades at $\lambda \gtrsim 8000$ \AA{}. We thus cut off the spectra in our analysis at $\lambda=8000$ \AA{} for spectra originating from  \aat{} and $\lambda=8200$ \AA{} for \mmt{}. 

Next, we flux calibrate our spectra using the SAGA g- and r-band photometry by assuming that the spectrum is representative of the full galaxy (i.e. assuming that there are no underlying population gradients) and applying the multiplicative conversion to reproduce the SAGA photometry from integrating the SAGA 
spectrum. This method is well-suited for our sample because the galaxies are generally small even compared to the relatively small \aat{} and \mmt{} fibers: the median on-sky effective radius of our sample is 1.2\arcsec{}, while the \aat{} and \mmt{} fibers are 2.1\arcsec{} and 1.5\arcsec{} in diameter, respectively. 
Because the g- and r-bands lie on different \aat{} spectrograph arms, we allow for different flux calibrations in g and in r for \aat{} spectra to correct for any discontinuities between the two arms 
that persisted beyond relative flux calibration. Finally, because the relative flux calibration is quite important for our metallicity measurements, we remove any \aat{} spectra where there a discontinuity of greater than 5\% across the spectrograph break after absolute flux calibration. 
%In \autoref{f:fluxcalibration} we show 
%example flux-calibrated SAGA spectra as compared to GAMA spectra that have been calibrated in their DR4.

We apply flux calibration to the SDSS spectra in the same way that we do for the SAGA AAT and 
MMT spectra. The flux calibration provided by the GAMA public data release are already 
calibrated consistently to our flux calibration and so we do not perform an additional 
flux calibration. For all spectra we correct for galactic extinction assuming a 
\cite{cardelli1989} extinction curve with an assumed $R_V=3.1$ and the galactic $A_V$ measured by
\cite{schlafly2011} at the position of each target. 


==> SAGAbgShared/spectra_second.tex <==
\subsection{The SAGA Spectra}
We use the flux-calibrated spectra detailed in \citetalias{otherpaper}
to measure the line fluxes of our SAGA galaxies. For completeness, we will briefly recount the flux calibration method here, but direct the reader to \citetalias{otherpaper} for a more detailed account of the calibration method.

The \aat{} and \mmt{} spectra taken by the SAGA survey require flux calibration in order to measure line fluxes; these spectra have already been relatively flux calibrated and so here we restrict our processing to an absolute flux calibration. The relative flux calibration of the spectra often degrades at 
$\lambda \gtrsim 8000$ \AA{} and $\lambda \gtrsim 8200$ \AA{} for the 
\aat{} and \mmt{} spectra, respectively, and so we restrict our flux measurements to those lines with an observed-frame wavelength of less than this cutoff value. We additionally remove any \aat{} spectra whose relative flux calibration changes by more than 5\% in the spectra region of the break between the blue and red arms of the instrument.

Our absolute flux calibration is calculated to match the observed $g$ and $r$ band SAGA photometry. This approach assumes that the (fiber) spectrum is representative of the full galaxy spectral energy distribution -- in other words, we assume that there is no change in the SED beyond the spatial extent of the fiber. We recompute the absolute flux calibration of the SDSS spectra in our sample, but find that our absolute flux calibration is consistent with the flux calibration of the GAMA team to around 5\%. We thus do not redo the flux calibration of the GAMA spectra.

We additionally correct for galactic extinction assuming a 
\cite{cardelli1989} extinction curve where $R_V=3.1$ and the galactic
extinction as measured by \cite{schlafly2011} at the 
coordinates of each galaxy.


==> SAGAbgShared/targeting_first.tex <==
\subsection{Photometric Selection}\label{s:sample:photometric}
The photometric targeting of the SAGA survey is designed to completely span the 
range of photometric properties occupied by the SAGA satellites, low-mass (\logmstar[$\lesssim 10$]) galaxies at $z\lesssim 0.02$. The exact nature of the 
photometric targeting has changed with time. As the survey progressed, the region of photometric space that encloses the set of SAGA satellites became more well-understood, allowing for stricter photometric cuts (see, for example, the cuts applied in \citealt{geha2012} as opposed to those in \citealt{mao2021}). Because the survey was completed in a host-by-host fashion, this means that the effective selection function may vary significantly between host fields. The spatial coverage of targets outside of the host virial radius is also significantly lower than inside the virial radius in a host-dependent manner.
Additionally, around half of the survey's spectroscopic resources were devoted to ``exploratory'' spectra: 
spectra of galaxies from the targeting catalog that did not meet the survey's criteria to be a main science target at the time of observation. 

In principle, the targeting function for SAGA background galaxies is a function of host and observation time in addition to the more explicit cuts on photometric properties. Because we are interested \textit{only} in the galaxies not associated with the SAGA hosts, however, we argue below that it is sufficient to characterize the realized aggregate selection function of the SAGA background galaxies. 

Having excluded the satellites of the SAGA hosts, the SAGA host fields can be considered to be random fields. The fact that some fields have a higher 
spatial completeness or a larger on-sky area should then not bias the characteristics of the aggregate sample except in cases of significant cosmic variance. Similarly, since there should be no differences in the population of galaxies between random field A (which corresponds, say, to host NSA 157300) and random field B (which may correspond to host PGC 66934), there should also be no difference -- modulo cosmic variation -- between targeting each random field with somewhat different photometric cuts and targeting both fields with the  average photometric cuts as weighted by number of spectra obtained using each selection function.

Taking this aggregate approach allows us to characterize the sample by its effective
photometric selection, which we will quantify as the fraction of galaxies that 
have received a ``first round'' redshift. We define the ``first round'' of redshifts as those that originate from SDSS, GAMA (AAT), or AAT/MMT observations. We note that this 
effective selection is different from but not discrepant with the SAGA photometric selections
that have been presented in~\cite{geha2012} and \cite{mao2021}. We will defer a 
full characterization of this aggregate selection function and its impact on the present sample to 
\autoref{s:modeling}, but to acquaint the reader with the sample at hand we 
show in \autoref{f:zlogm} the distribution of the sample over redshift and
 stellar mass. To orient the reader in this space, we show the stellar mass
that would correspond to an apparent magnitude of $m_r=19.8$ for a galaxy with 
a restframe color of $(g-r)=0.3$ using our color-mass relation as an orange curve. 
This apparent magnitude is roughly equal to the limiting magnitude of most field in the
Galaxy Mass and Assembly (GAMA) survey \citep{driver2009}.

%In particular, one can
%see the impact of targeting guided by these photometric selections in the sharp %decrease in first-round redshift fraction for redder ($g-r>0.95$, middle and right %panel groups) and high surface brightness (left and right panel groups) galaxies. 

At this juncture, we would like to take the opportunity to explicitly state the general approach that we utilize in this work. The SAGA photometric selection has been constructed to be complete at $z<0.035$ \citep{mao2021}, but the present sample will extend to $z=0.21$. We are thus functionally incomplete in a way that is quite sensitive the photometric property of the galaxies in question. Our focus on the star-forming sample does ameliorate this incompleteness, but we will build our models around the idea our sample in incomplete, and that we can quantify our incompleteness relative to some ``most complete'' subset. We will return to this idea more quantitatively in \autoref{s:modeling} when we build a model to understand the physical evolution of our observed samples.



==> SAGAbgShared/targeting_second.tex <==
\subsection{Photometric Selection}\label{s:sample:photometric}
As in \citetalias{otherpaper}, we consider the realized targeting selection of the SAGA spectroscopic campaign rather 
than attempting to reproduce its construction. 
This is because the spectroscopic targeting priorities have changed 
significantly over the lifetime of the survey in order to increase the purity of MW-like satellite selection \citep{geha2017, mao2021}. Furthermore, because the SAGA satellites themselves are excluded from the sample, we argue that it is appropriate to 
approximate the SAGA host fields as random fields. By definition and modulo cosmic variation, the population of galaxies from which the sample of galaxies in each of the SAGA host fields should therefore be the same. Thus, there should also be no difference between targeting each random field with somewhat different photometric cuts and targeting all fields with the average photometric cuts as weighted by number of spectra obtained using each selection function. Taking this approach allows us to estimate the relative completeness of the \sagabg{} sample via the effective aggregate photometric selection; we will defer a complete characterization of this selection function to \autoref{s:modeling:observational}.


Finally, as we stressed in \citetalias{otherpaper}, we note here that our approach to modeling the SAGA sample is based upon relative rather than absolute completeness. That is, we will build our models on the idea that the sample is most complete at our lowest redshift, and that we can quantify our redshift-dependent incompleteness using our knowledge of our selection criteria and our most complete subset at low redshift.
